Embedded Human-Centered Data Science in a Graduate Programming Course: A Framework and Case Study

As AI and data-driven systems pervade practice, there is an imperative for instructors to embed societal impact and ethics content into computing courses. In response, we present the Human-Centered Education for Learning in Information and eXplainable Computing (HELIX) framework for information science programs, organized around three iterative pillars - knowledge building, decision-making, and empowerment - with concrete actions for instructors and students. We applied the framework in a graduate, introductory programming course using readings, algorithmic design activities, and scenario-based reflections. We present a pilot implementation of this framework to examine changes in students' (n=22) knowledge acquisition, decision-making processes, and self-reflection regarding human-centered perspectives in data science. We release an anonymized materials kit (survey, assignments, analysis code) to support adoption. We discuss design tensions (workload, assessment, relevance to diverse information science learners) and provide guidelines for integrating human-centered content without overwhelming technical outcomes. Findings suggest that the HELIX Framework is feasible in information science contexts and future work should use comparative survey assessment to strengthen causal inferences.

==> PLOs.tex <==
\begin{itemize}
    \item UWash Master of Info Sci has AI ethics in AI stream but NO mention of ethics or human-centeredness in data science stream. Some PLOs %https://ischool.uw.edu/programs/mlis/curriculum/student-learning-outcomes
    \item UMich Master of Sci in IS has Big Data Analytics stream with NO mention of ethics or human-centeredness
    \item UWisconsin has PLOs: https://ischool.wisc.edu/wp-content/uploads/sites/1931/2022/06/MSHandbook2022.pdf with HC principles
    \item Cornell has data science ``focus area" but no mention of ethics or human-centeredness
    \item CMU has no learning outcomes, minimal HC content in course offerings
    \item Dalhousie (new in 2025) has no HC concepts on website
    \item Edinburgh Napier has no PLOs, HC
    \item Western has MLIS with learning outcomes (HC) %https://www.fims.uwo.ca/programs/graduate_programs/master_of_library_and_information_science/goals_and_learning_outcomes.html
    \item Fordham Uni has PLOs for Bachelor Info Tech degree %https://www.fordham.edu/academics/departments/computer-and-information-science/academic-programs/undergraduate-programs/information-technology-degree/learning-outcomes-for-bais/
    \item Illinois has PLOs %https://ischool.illinois.edu/academics/graduate/ms-library-and-information-science/learning-outcomes
    \item North Texas has PLOs for each degree but no HC mention %https://informationscience.unt.edu/about/mission.html
    \item McGill has PLOs but no HC mention %https://www.mcgill.ca/sis/programs/mist
    \item Dominican has PLOs, less data science related %https://www.dom.edu/academics/majors-programs/informatics/learning-goals-and-outcomes
    \item Karkstad teaches AI but no PLOs/HC
\end{itemize}


Trends in PLOs:

\begin{enumerate}
    \item Understanding information practices, new technology, information literacy, information access, changing practices, multi-media management, data management
    \item Leadership, user-centered society, responsibility, public good, equality, societal impact, legal/ethical principles
    \item Continued critical assessment, professionalism, professional development, interdisciplinary, intellectual growth, ongoing learning
\end{enumerate}
